MAGVIT: Masked Generative Video Transformer

We introduce the MAsked Generative VIdeo Transformer, MAGVIT, to tackle various video synthesis tasks with a single model. We introduce a 3D tokenizer to quantize a video into spatial-temporal visual tokens and propose an embedding method for masked video token modeling to facilitate multi-task learning. We conduct extensive experiments to demonstrate the quality, efficiency, and flexibility of MAGVIT. Our experiments show that (i) MAGVIT performs favorably against state-of-the-art approaches and establishes the best-published FVD on three video generation benchmarks, including the challenging Kinetics-600. (ii) MAGVIT outperforms existing methods in inference time by two orders of magnitude against diffusion models and by 60x against autoregressive models. (iii) A single MAGVIT model supports ten diverse generation tasks and generalizes across videos from different visual domains. The source code and trained models will be released to the public at https://magvit.cs.cmu.edu.

==> sections/3_method_backup.tex <==

% Our goal is to design a new video synthesis paradigm which enables a diverse set of generation tasks with a single model.
% \lu{we achieve this by [1 sentence]. As illustrate in \cref{fig:pipeline}, explain the high-level idea of your method [3-5] sentences. Here try to stay with natural language for better understanding. Below you gonna do formal description.}.
% For the likelihood model $\mathcal{G}$, we propose to learn a bidirectional transformer with \textit{\methodfullname{}} (\methodname).




\subsubsection{Background}

%This section discusses the conditional mask modeling used in the multi-task training.

Let $\rmV \in \sR^{T \times H \times W \times 3}$ be a video clip of $T$ frames each with $H \times W$ pixels.
The VQ encoder learned in the first stage tokenizes the video $f_\gT: \rmV \rightarrow \rmZ \in \sC^{t \times h \times w}$, where $\sZ$ is the codebook of integer indices.

Prior works~\cite{chang2022maskgit,gu2022vector,gupta2022maskvit} apply MTM to the 1D sequence $\rvz$ flattened from $\rmZ$. Let $\rvm \in \{\varnothing, \mask \}^{thw \times 1}$ denote a binary mask for $\rvz$, and $\rvz_{\overline{\rvm}}=g_\gM(\rvz, \rvm)$ be the sequence after applying the mask $\rvm$ to $\rvz$, in which each element is given by:
\begin{align}
g_\gM(\rvz, \rvm)_i =  
\begin{cases}
\mask &\text{if } \ervm_i = \mask \\
\ervz_i & \text{otherwise}
\end{cases}
\end{align}

A bi-directional transformer~\cite{devlin2019bert}, parameterized by $\theta$, is trained with MTM, with the objective to minimize the cross-entropy between the predicted token and the ground-truth token at each masked position.
\begin{equation}
\Ls = \mathop{\E}\limits_{\rvz \sim \gD} \Big[\sum_{\ervm_i \ne \varnothing} -\log p_\theta (z_i| \rvz_{\overline{\rvm}}) \Big]
\end{equation}

During training, $\rvm$ is uniformly sampled in which the fraction of masked position (or the mask ratio) is parameterized by a cosine function $\gamma(\cdot) \in (0, 1]$~\cite{chang2022maskgit}.
%according to a dynamic ratio of \mask elements, which follows a schedule function $\gamma(r) \in (0, 1]$~\cite{chang2022maskgit}.
% For positions where $\ermM_i$ equals \mask, a special mask token is used to replace the token $\ermZ_i$.
% $f_{\gT}^{-1}: \sC^{t \times h \times w} \rightarrow \sR^{T \times H \times W \times 3}$ is the decoder that generates the video clip from discrete tokens.

At inference, the model $\theta$ is used to generate token sequences by the non-autoregressive decoding algorithm~\cite{ghazvininejad2019mask,chang2022maskgit}. For example, MaskGIT's parallel decoding is given by:
\begin{algorithmic}[1]
{\small
\Require{$\rvm = \vzero$, $T$, $\theta$, $n = t\times h \times w$}
\For {$q \gets \frac{1}{T}, \frac{2}{T}, \cdots $ to $1$}
\State $\hat{\ervz}_{i} \sim p_{\theta}(\ervz_i| \rvz_{\bar{\rvm}})$, $\forall i$ where $m_i=$ \mask
\State $\text{topk} \gets \{j | j \in \arg\mathrm{topk}_{i} (p_{\theta}(\ervz_i| \rvz_{\bar{\rvm}})), k= \lceil \gamma(q) n \rceil\}$
\State $\rvm^{(t)} \gets \rvm^{(t-1)} + \vone()$
\EndFor
}
\end{algorithmic}

The conditioned signals, \eg, a class or a text description, are modeled as additional tokens $\rvc$ prepended to the masked sequence $\rvz_{\overline{\rvm}}$ to model the conditional probability $p_\theta(z_i | \rvz_{\overline{\rvm}}, \rvc)$. 








\subsubsection{Conditioned Mask Training}

The prefix condition works when condition shares no overlap with the $\rmZ$. It has three disadvantes to model condition in which the condition $\rmI$ a a subset of the input $\rmV$. In this paper, we call them interior condition:

% We can divide possible condition inputs for video generation tasks into two types:
% \begin{itemize}[nosep, leftmargin=*]
% \item exterior condition $E \nsubseteq V$, such as cross-modal  an action class or a text description.
% \item interior condition $I \subseteq V$, such as a frame or a spatial region.
% \end{itemize}

In multi-task generation, the model is given a task ID, a conditioned video clip $\rvv$ 
\cite{han2022show} mask at the latent space.

Unlike prior works that treat $\rvz$ as a 1D sequence, we retain the 3D dimension and use $\ervz^{(x,y,z)}$ to index the token at time $x$ and spatial location $(y,z)$ in the latent space.

Given the video token, the training objective of masked modeling in. 
Section visits autoregressive training.

% Existing masking method can be understood as:
% $$\rmZ_{\overline{\rmM}} =  \rmM \odot \rmZ + (1-\rmM) \mask$$
% $$\rmZ = P(Z |\rmZ_{\overline{\rmM}}) = \prod_{m_i=1} P_\theta(\ermZ_i | \rmZ_{\overline{\rmM}})$$

In our problem, we introduce a new mask which can take any token in the codebook. Compared to the conventional binary mask, its element can take any value to embed interior condition.


conditioned video $\rmV_{\text{cond}}$ which includes subset pixel of $\rmV$.

\lu{explain how to compute M}

Given the conditional mask, the loss become:



The proposed interior mask is conditional:
\begin{align}
\rmM \sim P_M(\rmV_{\text{cond}}, \text{PMT}_{\text{task}})
\end{align}
% $$\rmZ_{\overline{\rmM}} =  \rmM \odot \rmZ + (1-\rmM) \rmZ_{\text{cond}}$$

{
\small
\begin{align}
\Ls_{\text{MLM}}(\rmZ) = - \mathop{\mathbb{E}} \limits_{\rmM' \sim p_M'} \Big[ \sum_{\forall i} \log p_\theta (\ermZ_i | \rmM'(\rmZ)) \Big] \\
= - \mathop{\mathbb{E}} \limits_{\rmM' \sim p_M'} \Big[ 
\underbrace{\sum_{M_i=0} \log p_\theta (\ermZ_i | \rmV_{\text{cond}})}_{\text{refine}} 
+ \underbrace{\sum_{M_i \ne 0} \log p_\theta (\ermZ_i | \rmM'(\rmZ)) \Big]}_{prediction}
% \hat{\rmZ} &= P(Z|\rmZ_{\overline{\rmM}}) = \prod_{\forall i} P_\theta(\ermZ_i | \rmZ_{\overline{\rmM}}) \\
% &= \prod_{z_i \in \rmZ_{\text{cond}}} P_\theta(\ermZ_i | \rmZ_{\text{cond}}) *   \prod_{z_i \notin \rmZ_{\text{cond}}} P_\theta(\ermZ_i | \rmZ_{\text{cond}})\\
\end{align}
}

$$\rmZ_{\text{cond}} = f_\gT (\rmV_\text{cond})$$

During decoding, \lu{explain}


\subsection{\methodfullname}
\label{sec:ict}

We can divide possible condition inputs for video generation tasks into two types:
\begin{itemize}[nosep, leftmargin=*]
\item exterior condition $E \nsubseteq V$, such as cross-modal  an action class or a text description.
\item interior condition $I \subseteq V$, such as a frame or a spatial region.
\end{itemize}

We focus on a universal modeling of $I$, while we assume $E$ can be represented as a single embedding vector for simplicity.
We define the format of $I$ as a padded video $V_I \in \mathbb{R}^{T \times H \times W \times 3}$ with a binary mask $V_M$ indicating valid condition pixels.
We can tokenize it into condition code $C_I = \mathit{select}(\mathcal{T}(V_I))$, where the $\mathit{select}$ function only keeps valid tokens and replaces tokens whose patches are pure paddings with the special \texttt{[MASK]} token. 
The bottom left of \cref{fig:pipeline} illustrates this tokenization process.
% It is worth noting that a valid condition token is likely different from the corresponding token in the full code, as discussed in \cref{sec:tok}.
% TODO: this may change later, e.g., no replacement of [MASK], but this is what we are doing now

\methodname{} is a strict extension of the \textit{Masked Visual Token Modeling} (MVTM) training objective 
%in MaskGIT~\cite{chang2022maskgit}.
MVTM only replaces uniformly sampled tokens with the \texttt{[MASK]} token, which is a special case for \methodname{} with $I = \varnothing$.
\methodname{} replaces custom-selected tokens with the corresponding condition tokens if valid.

During training, \methodname{} uses a replacer function $\mathcal{R}$ to create model inputs $\tilde{C} = \mathcal{R}(C; C_I, \gamma(r))$, where $\gamma(r) \in (0, 1]$ is a dynamically sampled replacement rate.
The operation of $\mathcal{R}$ is parameterized by a per-token score $f(S) \in \mathbb{R}^{t \times h \times w}$.
Tokens in $C$ corresponding to the $\lceil \gamma(r)thw \rceil$ lowest entries in $f(S)$ are replaced by tokens from $C_I$.
$S \sim \mathit{uniform}(0, 1)$ during training.
$f$ is an optional task specific transformation, such as adding a fixed bias.

The transformer model $\mathcal{G}$ learns a reverse function of $\mathcal{R}$ to recover the original code $C$. The training objective is to minimize the negative log-likelihood of each token the full code:
\begin{equation}
\mathcal{L}_{\methodname} = - \mathbb{E}_{C \in \mathcal{T}(\mathbf{D})}[\sum_{x, y, z}\log P(C^{x, y, z} \mid \tilde{C})]
\end{equation}
where $\mathbf{D}$ is the training data set.

Concretely, we feed the training inputs $\tilde{C}$ into a multi-layer bidirectional transformer to predict the probabilities $P(C^{(x, y, z)} \mid \tilde{C})$ for each token.
The negative log-likelihood is computed as the cross-entropy between each ground-truth token and predicted token.


what is the prefix condition.

%-----------------------------------------------------------------------------------
\subsection{Conditional Iterative Generation}
\label{sec:cid}
Following the extension from MVTM to \methodname{}, the sampling procedure of \modelname{} also extends the iterative decoding algorithm in MaskGIT~\cite{chang2022maskgit}.
MaskGIT decoding gradually reduces the number of \texttt{[MASK]} tokens in the code through iterations.
\modelname{} conditional iterative generation gradually reduces the number of condition tokens that were replaced into the code.

Given the condition code $C_I$ and optionally $c_E$, we iterate between the replacer $\mathcal{R}$ and the transformer $\mathcal{G}$ for $N$ steps, with a decreasing replacement rate $\gamma(r)$.
The dashed line in \cref{fig:pipeline} shows the feedback path for this sampling loop, in addition to the training path.

We define $\gamma(r)$ as a monotonically decreasing function where $\gamma(0) = 1$ and $\gamma(1) \rightarrow 0$.
The overall likelihood of the generated code can be given as
\begin{equation}
    \begin{aligned}
    P(C \mid C_I, c_E) &= \\
    \prod_{i=1}^N P_\mathcal{G}(C_i &\mid \tilde{C}_i; c_E) P_\mathcal{R}(\tilde{C}_i \mid C_{i - 1}; C_I, \gamma(\frac{i - 1}{N}))
    \end{aligned}
\end{equation}

In practice, once a token is not replaced by $\mathcal{R}$ for the first time, we keep it fixed from then on.
This is done by overriding the distribution of these tokens to $P(C_{i-1}^{(x, y, z)})=1$ before sampling $C_i$ from $P_\mathcal{G}$.
The sampling likelihood then becomes the raw replacement score $S$ for $\mathcal{R}$ in the next iteration.
This dependency of $S$ is the only difference between a training step and an inference step, minimizing the train-test discrepancy. 
TODO: figure of generation process

The transformer $\mathcal{G}$ trained with \methodname{} predicts all tokens at each iteration, so minimally $N = 1$ is sufficient.
In practice, since the model only predicts the marginal probability of each token, iterative refinement has been proved to improve generation quality \cite{chang2022maskgit, gupta2022maskvit}.
As $N \ll thw$, this iterative decoding is orders-of-magnitude faster than autoregressive counterparts \cite{ge2022long} which only decode one token at a time.
This is also much faster than continuous diffusion methods \cite{ho2022video}, where detailed comparisons are provided in \cref{sec:efficiency}.

\subsection{Multi-task Conditional Modeling}
\label{sec:mt}
Our \methodname{} offers a universal modeling of generation tasks with interior condition.
Before this, there have been several ways to train a single conditional generation task.

For a single generation task, \methodname{} is just yet another alternative method.
The most straight forward way would be adding prefix condition tokens when training with MVTM, as denoted in 

A bidirectional transformer trained with MVTM inherently has the capability to handle different type of inputs in the latent space, presented as different masking of the full code $C$.
However, $C$ is unavailable at inference time and the actual condition code $C_I$ can be different.


MVTM + extra cond
MVTM + fixed cond
\methodname{}



\subsection{Spatiotemporal Tokenization}
\label{sec:tok}


$C_I^{a, b, c} = C^{a, b, c}$ where $M_I^{x, y, z} > 0 \forall x \in [a\frac{T}{t}, (a+1)\frac{T}{t}], y \in [b\frac{H}{h}, (b+1)\frac{H}{h}], z \in [c\frac{W}{w}, (c+1)\frac{W}{w}]$

\begin{equation}
    C_M^{(x, y, z)} = \left \{
    \begin{aligned}
        1,& \text{if} \textstyle\sum_{x=a\frac{T}{t}}^{(a+1)\frac{T}{t}}\sum_{y=b\frac{H}{h}}^{(b+1)\frac{H}{h}}\sum_{z=c\frac{W}{w}}^{(c+1)\frac{W}{w}}M_I^{(x, y, z)} = \frac{THW}{thw} \\
        0,& \text{otherwise}
    \end{aligned}
    \right.
\end{equation}

==> sections/4_experiments_backup.tex <==
We conduct extensive experiments to verify the video generation quality, efficiency, and flexibility.
In \cref{sec:exp_quality}, we evaluate the generation fidelity on two tasks and three public benchmarks and report notable improvements (up to 77\%) over the previous best results.
We compare the inference efficiency with existing models in \cref{sec:exp_efficiency}, where our method has an orders-of-magnitude faster generation speed than autoregressive transformers and diffusion models.
In \cref{sec:exp_flexibility}, we demonstrate the multi-tasking flexibility on two datasets with our proposed set of tasks.
A single \modelname{} model is capable of all the tasks at good quality.
We also show qualitative results for each of the tasks.

\subsection{Experimental Setups}

\paragraph{Tokenizer}
We train 3D VQGAN models to quantize 16 video frames into $4 \times 16 \times 16$ visual tokens.
The parameters of the 3D VQGANs are initialized with the central inflation method from a 2D VQGAN trained on ImageNet~\cite{deng2009imagenet} in a corresponding setup.
Details of the model architecture and training protocol are provided in \cref{app:tok}.

\paragraph{Transformer}
We adopt the standard BERT~\cite{devlin2019bert} architecture without segment embeddings.
The input sequence includes the task prompt, the class prompt, and 1024 visual tokens.
Baseline models with prefix condition also have condition tokens which results in a longer sequence.
See \cref{app:tran} for details and hyperparameters.

\paragraph{Scale}
In the following experiments, we use two variants of \modelname{}, namely base (B) and large (L).
Both the tokenizer and the transformer are scaled accordingly.

\paragraph{Tasks}
We define a total of 10 different tasks for conditional video generation, as listed in \cref{tab:task}. Each task has its own set of condition pixels and corresponding conditional masks.
We provide the detailed definitions in \cref{app:task}.
\input{tables/tasks}

\paragraph{Metrics}
We use Fr\'echet Video Distance (FVD)~\cite{unterthiner2018towards} as the major evaluation metric as it captures motion feature and has a high relevance with human evaluation.
The feature for FVD calculation is extracted with an I3D model trained on Kinetics-400~\cite{carreira2017quo}.
We report Inception Score (IS)~\cite{saito2020train} on the UCF-101 dataset, which is calculated with a C3D~\cite{tran2015learning} model trained on UCF-101.
We also report image quality metrics including Peak Signal-to-noise Ratio (PSNR), Structural Similarity Index Measure (SSIM)~\cite{wang2004image} and Learned Perceptual Image Patch Similarity (LPIPS)~\cite{zhang2018unreasonable}.
We sample videos from the dataset without replacement to form the real distribution in FVD and the condition inputs for the model.
We report the mean and standard deviation for each metric calculated with 4 runs.

\subsection{Single-Task Generation}
\label{sec:exp_quality}
We train \modelname{} with a single task to compare with prior works on standard benchmarks.

\paragraph{Class-conditional Generation (CG)}
\input{tables/cg}
In this task, the model is given a class prompt to generate a full video.
Since no interior condition is given, the training objective degrades to the conventional MTM.
We adopt the broadly used UCF-101~\cite{soomro2012ucf101} dataset to evaluate the CG performance.
UCF-101 consists of 101 classes and 9.5k videos for training and 3.8k videos for evaluation.
The benchmark evaluates $16 \times 128 \times 128$ videos and calculates FVD with 10k samples against the training set.
As shown in \cref{tab:ucf}, \modelname{} surpasses previous best FVD and IS values even with the base setup.
Our model improves the FVD metric by 77\%, setting a new state of the art at 76 from previous best 332.
We also increase IS by 13\% to 89.27, which gets very close to the IS of real data 91.36.

\paragraph{Frame Prediction (FP)}
\input{tables/fp}
In this task, the model is given a few frames at the beginning to generate the remaining frames.
The last condition frame is replicated to form the condition video.
We evaluate the FP task on the standard BAIR~\cite{ebert2017self, unterthiner2018towards} dataset and the large-scale Kinetics-600~\cite{carreira2018short} dataset.
BAIR contains 43k videos for training and 256 videos for evaluation, where the observer view is used for this benchmark.
The videos are at $64 \times 64$ resolution and the first frame is provided as condition.
Kinetics-600 contains 384k videos for training and 29k videos for evaluation.
We follow the standard practice~\cite{clark2019adversarial} in using the first 5 frames as condition.
We train \modelname{} to generate $16 \times 64 \times 64$ videos on BAIR and $16 \times 128 \times 128$ videos on Kinetics-600.
Following prior works, FVD for both datasets are calculated with $16 \times 64 \times 64$ videos against the evaluation set, with 256 $\times$ 100 samples for BAIR and 50000 samples for Kinetics-600.

As shown in \cref{tab:bairk600}, \modelname{} sets new state-of-the-art results on both FP benchmarks, with a 39\% improvement on Kinetics-600 to FVD 9.9 and a 18\% improvement on BAIR to FVD 69.
We also identify an issue with the existing BAIR evaluation protocol which only utilizes the first 16 frames of the 256 test videos.
The real distribution for FVD is highly biased with such few examples~\cite{unterthiner2018towards}.
We propose to use uniformly sampled 16-frame clips from the 256 30-frame videos, which results in $256 \times 15 = 3840$ possible clips.
Under this new protocol, \modelname{} achieves FVD 32, which is more aligned with training set performance as detailed in \cref{app:bair}. 

\subsection{Inference Efficiency}
\label{sec:exp_efficiency}
\input{tables/efficiency}
We report the number of decoding steps and total decoding FLOPs of recent video generation models, as listed in \cref{tab:efficiency}.
The measured computation cost are based on the generation of a $16 \times 128 \times 128$ video.
We also include the number of tokens for transformer-based models.
For autoregressive models which decode one token at a time, the number of steps equals the number of tokens, which is around 1024-8192.
For diffusion models, the number of steps is defined by the diffusion process, which lies within 256-1000.
For bidirectional transformers, the number of steps is a hyperparameter at inference time, which is usually chosen between 12-64.
The number of tokens is determined by the compression ratio of the tokenizer.
3D tokenizers can compress both spatially and temporally, while 2D cannot to temporal compression.
\lijun{analysis when table is ready}.

\subsection{Multi-task Video Synthesis}
\label{sec:exp_flexibility}
We train multi-task \modelname{} models to demonstrate its flexibility and generic modeling capability.
We propose two benchmarks for this purpose, with 8 tasks on the unlabeled BAIR dataset and 10 tasks on the Something-Something-v2 (SSV2) action recognition dataset.

\paragraph{BAIR 8-task}
\input{tables/mt_bair}
Since BAIR does not have class labels, CG and CFP tasks are not applicable.
We first perform multi-task evaluation on BAIR with the remaining 8 tasks.
We use the FVD metric with the new evaluation protocol for each task and calculate an aggregated average score.
We use two single-task models as baselines, one for unconditional generation (UNC) and one for frame prediction (FP).
The unconditional model does not see any condition tokens during training, so its performance can roughly reflect the distributional difference between condition tokens of each task and the full tokens.
The frame prediction model corresponds to the commonly used benchmark on BAIR.

The BAIR 8-task results are shown in \cref{tab:mt_bair}.
The UNC model achieves an average score of 150.6, where vertical and horizontal outpainting tasks are the easiest to generalize to.
Dynamic outpainting and inpainting are the hardest tasks for this model, as their condition tokens are completely unseen due to the continuously moving condition regions.
The FP model performs well in the frame interpolation task which is similar to its training task.
But it performs way worse than the UNC model in static outpainting and inpainting tasks, leading to an average score of 201.1.
This demonstrates the poor generalizability of a specialized single task model that the literature has been focusing on.

The MT8 model is trained with all 8 tasks to achieve real multi-tasking capability.
Even with the same amount of parameters, it easily performs well on all of them.
Compared with the UNC model, MT8 performs significantly better on every task, indicating the importance of multi-task training over simple unconditional modeling.
Even compared with the specialized FP model, MT8 demonstrates a matching performance in the frame prediction task and is much better in the others.
The MT8 base model achieves an average score of 32.8 for the FVD over 8 tasks.
Scaling to the large model can further bring the average score down to 22.8.
For the two MT8 models, FP and FI appear to be harder than the others.

\paragraph{SSV2 10-task}
\input{tables/mt_ssv2}
We propose to use a new dataset, Something-Something-v2 (SSV2), for the evaluation of multi-task video synthesis.
SSV2 contains 169k videos for training and 25k videos for evaluation in 174 classes.
Its videos are about human performing pre-defined basic actions with everyday objects.
The models have to learn to synthesize complex scenes and actions on SSV2, which makes it a more challenging benchmark than the commonly used BAIR dataset.

We evaluate the multi-task capability on SSV2 dataset with all 10 tasks, 2 of which use the class labels.
We calculate the FVD metric with 50000 samples against the training set for the CG task and against the validation task for the other tasks.
We use a single task model trained with CG as the baseline.
As shown in \cref{tab:ssv2}, the SSV2 10-task results show a similar pattern as BAIR 8-task.
For the CG model, OPV and OPH remain the easiest while OPD and IPD appear to be the hardest.
The baseline average score is 258.8, with a CG FVD of 107.7.
The 10-task model achieves an average score of 45.6, with huge improvements on all 9 new tasks compared with the CG model.
The FVD distribution among the 10 tasks is reversely relevant to the proportion of condition pixels, with CG (0\%) being the most difficult and inpainting (75\%) the easiest.
Scaling to the large model can further improve the average score to 29.9.

\subsection{Ablation Study}

\paragraph{Condition method on single task}
% \lijun{also: misalignment between training tokens and inference tokens which come from only condition region}

\paragraph{Condition method on multi-task}

\paragraph{2D or 3D tokenizer}
\label{sec:exp_tok}

\paragraph{tokenizer inflation}

\paragraph{Task token or not?}

\paragraph{autoregressive or bidirectional}


==> tables/efficiency.tex <==
% \begin{table}[!ht]
% \caption{Inference efficiency. \lijun{Needs verification}}
% \label{tab:efficiency}
% \centering
% \begin{tabular}{@{}lccc@{}}
% \toprule
% Method               & \makecell{Sequence\\length}    & \#Steps$\downarrow$ & Complexity $\downarrow$ \\ \midrule
% % CogVideo\cite{hong2022cogvideo} & 4096  & 4096 &   \\
% % CCVS\cite{le2021ccvs} & 4096  & 4096 &   \\
% % VideoGPT\cite{yan2021videogpt} & 8192 &    8192    &               \\
% % Transframer\cite{nash2022transframer} & 4096 &  4096  &                \\
% % N\"UWA\cite{wu2021n}  & 7056  & 7056  &        \\
% % RaMViD\cite{hoppe2022diffusion} & - &  1000   &   \\
% Video Diffusion\cite{ho2022video} & - & 256-512  & $\gO(THWK)$   \\ 
% TATS\cite{ge2022long} & 1024 & 1024 & $\gO(T^3H^3W^3)$ \\
% MaskViT\cite{gupta2022maskvit} & 4096 & 16-64  &    $\gO(T^2H^2W^2K)$           \\\midrule
% \modelname{}  (ours) &  1024 & 12  & $\gO(T^2H^2W^2K)$       \\ \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[tp]
\scriptsize
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
Method               & \makecell{Seq.\\length$\downarrow$}    & \# Steps$\downarrow$ & \makecell{Estimated\\Relative\\Runtime$\downarrow$} \\ \midrule
Video Diffusion\cite{ho2022video} & - & 256-512  & $\gg$250 \\ 
TATS\cite{ge2022long} & 1024 & 1024 & 60  \\
MaskViT\cite{gupta2022maskvit} & 4096 & 16-64  &   4-12   \\\midrule
\emph{\modelname}  (ours) &  \textbf{1024} & \textbf{12}  &   \textbf{1}   \\\bottomrule
\end{tabular}
\caption{\textbf{Comparison of key properties for inference efficiency.}}
\label{tab:efficiency}
\end{table}


==> tables/task_mask.tex <==
\begin{table}[!h]
\centering
\scriptsize
\begin{tabular}{@{}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{}}
\toprule
& CG & FP & CFP & FI & OPC & OPV & OPH & OPD  & IPC  & IPD \\ \midrule
Masked pixel & 100\% & 94\% & 94\% & 87\% & 75\% & 50\% & 50\% & 50\% & 25\% & 25\% \\
Masked token & 100\% & 75\% & 75\% & 50\% & 75\% & 50\% & 50\% & 50\% & 25\% & 25\% \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\caption{Proportions of masked pixels and tokens for each task.}
\label{tab:task_mask}
\vspace{-4mm}
\end{table}

==> tables/tasks.tex <==
\begin{table}[tp]
\centering
\scriptsize
\begin{tabular}{@{}lcc@{}}
\toprule
Task & \makecell{Condition Pixels} & \makecell{Fully Masked\\Input Tokens} \\ \midrule
\makecell[cl]{\textbf{CG}:\\Class-conditional\\Generation}   & \makecell{\includegraphics[width=.2\linewidth]{fg_vid}} & \makecell{\includegraphics[width=.2\linewidth]{fg_tok}}  \\
\makecell[cl]{\textbf{FP}:\\Frame\\Prediction}   & \makecell{\includegraphics[width=.2\linewidth]{fp_vid}} & \makecell{\includegraphics[width=.2\linewidth]{fp_tok}}  \\
\makecell[cl]{\textbf{CFP}:\\Class-conditional\\Frame Prediction}   & \makecell{\includegraphics[width=.2\linewidth]{fp_vid}} & \makecell{\includegraphics[width=.2\linewidth]{cfp_tok}}  \\
\makecell[cl]{\textbf{FI}:\\Frame\\Interpolation}   & \makecell{\includegraphics[width=.2\linewidth]{fi_vid}} & \makecell{\includegraphics[width=.2\linewidth]{fi_tok}}  \\
\makecell[cl]{\textbf{OPV}:\\Vertical\\Out Painting}   & \makecell{\includegraphics[width=.2\linewidth]{opv_vid}} & \makecell{\includegraphics[width=.2\linewidth]{opv_tok}}  \\
\makecell[cl]{\textbf{OPH}:\\Horizontal\\Outpainting}   & \makecell{\includegraphics[width=.2\linewidth]{oph_vid}} & \makecell{\includegraphics[width=.2\linewidth]{oph_tok}}  \\
\makecell[cl]{\textbf{OPC}:\\Central\\Out Painting}   & \makecell{\includegraphics[width=.2\linewidth]{opc_vid}} & \makecell{\includegraphics[width=.2\linewidth]{opc_tok}}  \\
\makecell[cl]{\textbf{OPD}:\\Dynamic\\Outpainting}   & \makecell{\includegraphics[width=.2\linewidth]{opd_vid}} & \makecell{\includegraphics[width=.2\linewidth]{opd_tok}}  \\
\makecell[cl]{\textbf{IPC}:\\Central\\Inpainting}   & \makecell{\includegraphics[width=.2\linewidth]{ipc_vid}} & \makecell{\includegraphics[width=.2\linewidth]{ipc_tok}}  \\
\makecell[cl]{\textbf{IPD}:\\Dynamic\\Inpainting}   & \makecell{\includegraphics[width=.2\linewidth]{ipd_vid}} & \makecell{\includegraphics[width=.2\linewidth]{ipd_tok}}  \\ \bottomrule
\end{tabular}
\caption{Task list with condition definition in pixel and token spaces. Condition pixels are in green, while paddings are in white. Condition tokens are in yellow and \mask tokens are in gray. An orange token indicates provided class index as prefix condition, while a white token indicates a \texttt{[NOCLASS]} token. \lu{The third column looks naive without much information. Consider making it two column table and add code for padding.}}
\label{tab:task}
\end{table}

==> tables/token2.tex <==
\begin{table}[!h]
\centering
\scriptsize
\begin{tabular}{l@{\hspace{6pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{7pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{7pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c}
\toprule
\multirow{2}{*}{VQ Tokenizer} & \multicolumn{3}{l}{From Scratch} & \multicolumn{6}{c}{ImageNet Initialization} \\
& P$\uparrow$ & S$\uparrow$ & L$\downarrow$ & P$\uparrow$ & S$\uparrow$  & L$\downarrow$ & P$\uparrow$ & S$\uparrow$ & L$\downarrow$ \\ \midrule
MaskGIT 2D  &
 21.4 & 0.667 & 0.139 & 21.5 & 0.685 & 0.114 & \multicolumn{3}{c}{-} \\
% TATS 3D & 
% 23.2 & 0.784 &  & \multicolumn{3}{c}{-}& \multicolumn{3}{c}{-} \\ 
\midrule
& & & & \multicolumn{3}{c}{Average} & \multicolumn{3}{c}{Central} \\
% \emph{\modelname{}} 3D-VQ-B & 
% 20.7 & 0.640 & 0.143 & 21.1 & 0.662 & 0.123 & 21.3 & 0.673 & 0.113 \\ 
\emph{\modelname{}} 3D-L &
21.8 & 0.690 & 0.113 & 21.9 & 0.697 & 0.103 & \textbf{22.0} & \textbf{0.701} & \textbf{0.099} \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\caption{\textbf{Image quality metrics of different tokenizers} on UCF-101 training set reconstruction.
P: PSNR, S: SSIM, L: LPIPS.
}
\label{tab:token_imquality}
\vspace{-4mm}
\end{table}

